EyeFormer: Predicting Personalized Scanpaths with Transformer-Guided Reinforcement Learning

From a visual perception perspective, modern graphical user interfaces (GUIs) comprise a complex graphics-rich two-dimensional visuospatial arrangement of text, images, and interactive objects such as buttons and menus. While existing models can accurately predict regions and objects that are likely to attract attention ``on average'', so far there is no scanpath model capable of predicting scanpaths for an individual. To close this gap, we introduce EyeFormer, which leverages a Transformer architecture as a policy network to guide a deep reinforcement learning algorithm that controls gaze locations. Our model has the unique capability of producing personalized predictions when given a few user scanpath samples. It can predict full scanpath information, including fixation positions and duration, across individuals and various stimulus types. Additionally, we demonstrate applications in GUI layout optimization driven by our model. Our software and models will be publicly available.

==> source/06a-quantitative_table.tex <==
\def\arraystretch{1}% 
\begin{table*}[t]
\scalebox{0.85}{\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccccccc}
\hline
\multirow{ 2}{*}{\textbf{Model}}  & \multirow{ 2}{*}{\textbf{DTW} $\downarrow$}  & \multirow{ 2}{*}{\textbf{TDE} $\downarrow$} & \multirow{ 2}{*}{\textbf{Eyenalysis} $\downarrow$} & \multirow{ 2}{*}{\textbf{DTWD} $\downarrow$} & \multicolumn{6}{|c}{\textbf{MultiMatch} $\uparrow$}  \\
 &  &  &   & &  \multicolumn{1}{|c}{\textbf{Shape}}   & \textbf{Direction}  &  \textbf{Length}   & \textbf{Position}   & \textbf{Duration}  & \textbf{Mean}  \\
\hline
Itti--Koch &   6.249 $\pm$ 0.986 &   0.150 $\pm$ 0.025 &     0.047 $\pm$ 0.028 &  --- &   0.861 &  0.721 & 0.819 &  0.746 &  ---&  --- \\ 
DeepGaze III Pretrained   &  7.906 $\pm$ 2.466  & 0.274 $\pm$ 0.061  &  0.124 $\pm$ 0.076 &  --- &  0.937 &  0.567 &  0.886&  0.746 &  ---&  --- \\ 
DeepGaze++ &  5.454  $\pm$ 1.078 & 0.149  $\pm$ 0.032 & 0.047  $\pm$ 0.026 &  --- &  0.907 & 0.708 &  0.906 &  0.773 &  ---&  --- \\ 
{PathGAN Pretrained}    &     4.719 $\pm$ 1.387 &    0.192 $\pm$ 0.049 &    0.072 $\pm$ 0.037&  ---  & 0.940 &  0.579 & 0.892 & 0.800   & --- & ---   \\ 
{PathGAN on UEyes}         &  4.754 $\pm$ 1.185 &   0.147 $\pm$ 0.048 &   0.048 $\pm$ 0.025 &  ---  & \bf 0.943 & 0.716 & 0.935 & 0.797 & --- & ---  \\ 
{PathGAN++ on UEyes}   &     4.559 $\pm$ 1.182 &     0.146 $\pm$ 0.037 &   0.044 $\pm$ 0.022 &   --- & \bf 0.943 & 0.706 & 0.933 & 0.807 &  --- & --- \\ 
{PathGAN w/ D on UEyes}     &  5.192 $\pm$ 1.422 &   0.204 $\pm$ 0.045 &   0.092 $\pm$ 0.038 & 6.431 $\pm$ 1.644 & 0.939 & 0.556 &  0.891 & 0.779 & 0.667 & 0.766 \\ 
{PathGAN++ w/ D on UEyes}        &  5.443 $\pm$ 1.466 &   0.202 $\pm$ 0.044 &   0.096 $\pm$ 0.043 & 6.667 $\pm$ 1.659  & 0.939 & 0.560 & 0.896  & 0.765  & 0.657 & 0.763 \\ 
{SaltiNet on UEyes}   &   7.042 $\pm$ 1.622 &   0.187 $\pm$ 0.057 &   0.063 $\pm$ 0.054 & 8.241 $\pm$ 1.487  &  0.907   &  0.715   &  0.897  &  0.691   &   0.579   &    0.758   \\
{UMSS on UEyes}   &   5.051 $\pm$ 1.592 &   0.155 $\pm$ 0.048 &   0.050 $\pm$ 0.026 & 6.495 $\pm$ 1.468  &  0.934   &  0.713   &  0.921  &  0.779   &   0.579   &    0.785   \\
{ScanGAN on UEyes}   &   4.815 $\pm$ 1.238   &   0.136 $\pm$ 0.034    &    0.040 $\pm$ 0.022 
  &   --      &   0.931    &    0.734   &   0.929    &    0.796    &   --   &  --          \\
{ScanDMM on UEyes}   &   5.085 $\pm$ 1.317   &    0.138  $\pm$  0.037   &    0.043   $\pm$  0.027    &   --  &   0.931   &   0.729   &   0.928   &   0.784  &   --   &   --          \\
{Chen et al. Model on UEyes}  &   4.335  $\pm$  1.299   &   \bf 0.118   $\pm$  0.034   &   0.037  $\pm$  0.019     &    5.533 $\pm$ 1.250   &    0.939   &   0.725   &   0.926   &   0.823   &  0.720   &   0.827         \\
%\bf Ours   &   \bf  4.171 $\pm$ 1.056  &      0.122 $\pm$ 0.027 &  \bf  0.036 $\pm$ 0.018 &  \bf  5.096 $\pm$ 1.003 &  0.942   & \bf 0.745  &  \bf  0.940  &    0.821   &  \bf 0.748  &  \bf 0.839 \\ 
\bf Our Model   &   \bf 4.069  $\pm$  1.089    &   0.122  $\pm$  0.029   &   \bf 0.036  $\pm$  0.018   &  \bf  5.043  $\pm$  1.052  &   0.942    & \bf  0.748    &  \bf  0.940   &  \bf  0.825   &   \bf 0.750   & \bf  0.841    \\
\bottomrule
\end{tabular}
}

\caption{
    Quantitative scanpath evaluation, %on the \textit{UEyes} dataset, 
    with the mean $\pm$ \textit{STD} reported for each metric, where % Unless you want to write out `standard deviation reported'. -als
    ``Pretrained'' denotes testing via the pre-trained model  
    while ``on UEyes'' refers to fine-tuning with the eye-tracking dataset 
    (boldface highlights the best result column-wise; % FYI: I've changed the formatting such that you needn't end the table heading with a full stop.  Also, do you want/need to specify the units anywhere?  -als
    arrows indicate the importance relation's direction -- e.g., $\uparrow$ means ``higher is better'' -- and
    \ADD{``-'' is used for methods that, being unable to predict fixation duration, are excluded from metrics considering duration)}.
    % Our model demonstrates superior performance across all metrics, 
    % apart from \textit{Shape} in \textit{MultiMatch}, indicating that our model produces more accurate results.
}
\label{tbl:scanpaths_quantitative}
\end{table*}

==> source/06c-natural_scenes_quantitative_table.tex <==
\def\arraystretch{1}% 
\begin{table*}[t]
\scalebox{0.85}{\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccccccc}
\hline
\multirow{ 2}{*}{\textbf{Model}}  & \multirow{ 2}{*}{\textbf{DTW} $\downarrow$}  & \multirow{ 2}{*}{\textbf{TDE} $\downarrow$} & \multirow{ 2}{*}{\textbf{Eyenalysis} $\downarrow$} & \multirow{ 2}{*}{\textbf{DTWD} $\downarrow$} & \multicolumn{6}{|c}{\textbf{MultiMatch} $\uparrow$}  \\
 &  &  &   & &  \multicolumn{1}{|c}{\textbf{Shape}}   & \textbf{Direction}  &  \textbf{Length}   & \textbf{Position}   & \textbf{Duration}  & \textbf{Mean}  \\
\hline
Itti--Koch &   3.180 $\pm$ 0.756 &   0.176 $\pm$ 0.039 &     0.061 $\pm$ 0.027 &  --- &   0.859 &  0.653 & 0.811 &  0.748 &  ---&  --- \\ 
SGC   &  2.992 $\pm$ 1.067  & 0.194 $\pm$ 0.071  &  0.073 $\pm$ 0.046 &  --- &  0.922 &  0.652 &  0.890 &  0.768 &  ---&  --- \\ 
Wang et al.  &  3.798  $\pm$ 1.128 & 0.227  $\pm$ 0.073 & 0.096  $\pm$ 0.060 &  --- &  0.886 & 0.641 &  0.841 &  0.700 &  ---&  --- \\ 
Le Meur et al.   &    3.027 $\pm$ 0.797 &   0.160 $\pm$ 0.476 &    0.057 $\pm$ 0.028 &  ---  & 0.892 &  0.653 & 0.865 & 0.770   & --- & ---   \\ 
STAR-FC   &  3.375 $\pm$ 1.300 &   0.228 $\pm$ 0.091 &   0.090 $\pm$ 0.067 &  ---  & 0.936 & 0.662 & 0.920 & 0.734 & --- & ---  \\ 
SaltiNet   &    3.439 $\pm$ 0.861 &  0.191 $\pm$ 0.052 &   0.065 $\pm$ 0.032 &   3.860 $\pm$ 0.814 &  0.895 & 0.641 & 0.872 & 0.719 &  0.573 & 0.740 \\ 
PathGAN    &  5.300 $\pm$ 1.197 &   0.323 $\pm$ 0.073 &   0.142 $\pm$ 0.085 & 5.454 $\pm$ 1.167 & 0.935 & 0.577 &  0.924 & 0.608 & 0.679 & 0.745 \\ 
IOR-ROI   &  2.495 $\pm$ 0.809 &   0.160 $\pm$ 0.055 &   0.060 $\pm$ 0.039 & 2.955 $\pm$ 0.768  & 0.914 &  \bf 0.704 & 0.889  & 0.812  & 0.629 & 0.790 \\ 
Chen et al.  &   2.183  $\pm$  0.949   &   0.125   $\pm$  0.056  &   \bf 0.045  $\pm$  0.028     &  \bf 2.636 $\pm$ 0.865   &    0.944   &   0.653   &   0.924   &   0.847   & \bf 0.689   &  \bf 0.811         \\ 
\bf EyeFormer   &   \bf 2.181  $\pm$  0.911    &  \bf  0.119  $\pm$  0.048   &    0.048  $\pm$  0.030   &   3.231  $\pm$  0.975  &   \bf 0.950    &   0.668    &  \bf  0.936   &  \bf  0.850   &   0.617   &   0.804    \\
\bottomrule
\end{tabular}
}

\caption{
    Quantitative scanpath evaluation, %on the \textit{UEyes} dataset, 
    with the mean $\pm$ \textit{STD} reported for each metric (boldface highlights the best result column-wise; 
    arrows indicate the importance relation's direction -- e.g., $\uparrow$ means ``higher is better'' -- and
    \ADD{``-'' is used for methods that, being unable to predict fixation duration, are excluded from metrics considering duration)}.
    % EyeFormer demonstrates superior performance across all metrics, 
    % apart from \textit{Shape} in \textit{MultiMatch}, indicating that our model produces more accurate results.
}
\label{tbl:natural_scenes_scanpaths_quantitative}
\end{table*}

Itti--Koch~\cite{itti1998model}, SGC~\cite{sun2012what}, Wang et al.~\cite{wang2011simulating}, Le Meur et al.~\cite{lemeur2015saccadic}, STAR-FC~\cite{wloka2018active}, SaltiNet~\cite{assens2017saltinet}， PathGAN~\cite{Assens2018pathgan}, IOR-ROI~\cite{sun2021visual}, Chen et al.~\cite{chen2021predicting} 

==> source/07a-ComparisonFigures.tex <==
\setlength{\tabcolsep}{2pt}
\def\arraystretch{1}% 
\begin{figure*}[!]
\def\w{0.108\linewidth}
\def\ww{0.155\linewidth}
 \centering
\begin{tabular}{c *9c}
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \  \REVISION{Image}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/orig_images/eb06ec.jpg} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/orig_images/cd9e29.jpg} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/orig_images/46e638.jpg} &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/orig_images/5db7bc.jpg} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/orig_images/9aabba.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/orig_images/e7a5c0.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/orig_images/b4a27a.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/orig_images/c6a6d9.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \  \REVISION{GT}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/vertical_no_trans/eb06ec_kh044_gt.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/vertical_no_trans/cd9e29_kh005_gt.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/vertical_no_trans/46e638_kh028_gt.png} &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/horizontal_no_trans/5db7bc_kh005_gt.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/horizontal_no_trans/9aabba_kh012_gt.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/vertical_no_trans/e7a5c0_kh054_gt.png} &
\includegraphics[height=\w, trim=16 20 16 18, clip]{source/figures/horizontal_no_trans/b4a27a_kh004_gt.png} &
\includegraphics[height=\w, trim=18 20 18 18, clip]{source/figures/horizontal_no_trans/c6a6d9_kh004_gt.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \    \REVISION{Itti-Koch}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/comparison/99142_test_scanpath_Itti-Koch-based.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/comparison/dayama13 (3)_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_test_scanpath_Itti-Koch-based.png} 
\\
\bf \begin{turn}{90} 
\bf \   \REVISION{ DeepGaze++}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=16 10 0 5, clip]{source/figures/comparison/99142_test_scanpath_DeepGaze++.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/comparison/dayama13 (3)_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_test_scanpath_DeepGaze++.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_test_scanpath_DeepGaze++.png} 
\\
\bf \begin{turn}{90} 
\bf \ \   \REVISION{\begin{tabular}{@{}c@{}}PathGAN++ \\ on UEyes\end{tabular}}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/comparison/99142_test_scanpath_PathGAN++.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/comparison/dayama13 (3)_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_test_scanpath_PathGAN++.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_test_scanpath_PathGAN++.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \    \REVISION{\begin{tabular}{@{}c@{}}UMSS \\ on UEyes\end{tabular}} 
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/comparison/99142_test_scanpath_UMSS.png}&
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=10 10 10 0, clip]
{source/figures/comparison/dayama13 (3)_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_test_scanpath_UMSS.png}&
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_test_scanpath_UMSS.png}
\\
\bf \begin{turn}{90} 
\bf \  \REVISION{\begin{tabular}{@{}c@{}}ScanGAN \\ on UEyes\end{tabular}} 
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_kh004_scanpath_ScanGAN.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_kh005_scanpath_ScanGAN.png}  &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_kh012_scanpath_ScanGAN.png}  &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/comparison/99142_kh005_scanpath_ScanGAN.png}  &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_kh005_scanpath_ScanGAN.png}  &
\includegraphics[height=\w, trim=10 10 10 0, clip]
{source/figures/comparison/dayama13 (3)_kh005_scanpath_ScanGAN.png}  &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_kh004_scanpath_ScanGAN.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_kh004_scanpath_ScanGAN.png} 
\\
\bf \begin{turn}{90} 
\bf \  \REVISION{\begin{tabular}{@{}c@{}}ScanDMM \\ on UEyes\end{tabular}} 
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=16 10 0 5, clip]{source/figures/comparison/99142_test_scanpath_ScanDMM.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]
{source/figures/comparison/dayama13 (3)_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_test_scanpath_ScanDMM.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_test_scanpath_ScanDMM.png} &
\\
\bf \begin{turn}{90} 
\ \ \    \REVISION{\begin{tabular}{@{}c@{}} Chen et al.\\ on UEyes \end{tabular}}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/351_kh004_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/comparison/375_kh005_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/comparison/2308_kh012_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/comparison/99142_kh005_scanpath_ScanVQA.png}&
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/comparison/brilio_kh005_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/comparison/dayama13 (3)_kh005_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/comparison/ICWE_19_166_kh004_scanpath_ScanVQA.png}&
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/comparison/ICWE_19_392_kh004_scanpath_ScanVQA.png}
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \REVISION{\begin{tabular}{@{}c@{}}Ours\end{tabular}}
\end{turn} & 
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/vertical_no_trans/eb06ec_kh044_pred.png} &
\includegraphics[height=\w, trim=10 10 10 10, clip]{source/figures/vertical_no_trans/cd9e29_kh005_pred.png} &
\includegraphics[height=\w, trim=16 20 16 10, clip]{source/figures/vertical_no_trans/46e638_kh028_pred.png} &
\includegraphics[height=\w, trim=16 20 0 5, clip]{source/figures/horizontal_no_trans/5db7bc_kh005_pred.png} &
%\includegraphics[height=\w]{source/figures/comparison/AVI_14_132_test_scanpath_Itti-Koch-based.png} &
\includegraphics[height=\w, trim=10 10 10 5, clip]{source/figures/horizontal_no_trans/9aabba_kh012_pred.png} &
\includegraphics[height=\w, trim=10 10 10 0, clip]{source/figures/vertical_no_trans/e7a5c0_kh054_pred.png} &
\includegraphics[height=\w, trim=16 20 16 15, clip]{source/figures/horizontal_no_trans/b4a27a_kh004_pred.png} &
\includegraphics[height=\w, trim=18 20 18 15, clip]{source/figures/horizontal_no_trans/c6a6d9_kh004_pred.png} 
\\
\end{tabular}
\caption{
    \ADD{Qualitative comparison over a broad spectrum of scanpath models.
    Our model can predict more realistic scanpaths than others, also showing greater accuracy for individual fixation points. For fair comparison, all models apart from the Itti--Koch one (not deep-learning-based) and DeepGaze++ were trained on UEyes. This illustration presents the best baseline methods. }
}
\label{fig:scanpath_qualitative}
\end{figure*}

==> source/07b-ResultFigures.tex <==
\setlength{\tabcolsep}{1.5pt}
\def\arraystretch{0.8}% 
\begin{figure*}[h!]
\def\w{0.164\linewidth}
 \centering
\begin{tabular}{c *9c}
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ GT
\end{turn} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/0feea2_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/1a2fc7_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/6c8b71_kh054_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/46e638_kh028_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/598d81_kh044_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/5620ab_kh029_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/ab0c83_kh043_gt.png} &
\includegraphics[height=\w, trim=10 0 130 10, clip]{source/figures/horizontal_no_trans/5887a5_kh028_gt.png}  &
\includegraphics[height=\w, trim=55 0 80 0, clip]{source/figures/horizontal_no_trans/a8f275_kh028_gt.png}  
\\
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \  Prediction 
\end{turn} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/0feea2_kh037_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/1a2fc7_kh062_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/6c8b71_kh054_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/46e638_kh028_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/598d81_kh044_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/5620ab_kh029_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/ab0c83_kh043_pred.png} &
\includegraphics[height=\w, trim=0 0 130 0, clip]{source/figures/horizontal_no_trans/5887a5_kh028_pred.png}  &
\includegraphics[height=\w, trim=55 0 80 0, clip]{source/figures/horizontal_no_trans/a8f275_kh028_pred.png}
\\
\\
\end{tabular}
\def\w{0.158\linewidth}
 \centering
\begin{tabular}{c *9c}
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ GT
\end{turn} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/ab4d1f_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/cd9e29_kh005_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/d7cfda_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/e7a5c0_kh054_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/e18daf_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/eb06ec_kh044_gt.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/f285d7_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/b4a27a_kh004_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/c6a6d9_kh004_gt.png}
\\
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \   Prediction 
\end{turn} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/ab4d1f_kh037_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/cd9e29_kh005_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/d7cfda_kh012_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/e7a5c0_kh054_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/e18daf_kh012_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/eb06ec_kh044_pred.png} &
\includegraphics[height=\w]{source/figures/vertical_no_trans/f285d7_kh062_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/b4a27a_kh004_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/c6a6d9_kh004_pred.png}
\\
\\
\end{tabular}
\def\w{0.102\linewidth}
\begin{tabular}{c *6c}
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \ \  GT
\end{turn} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/0f1984_kh028_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/1c381f_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/2ffa4a_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/c8b126_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/d889b1_kh048_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/9aabba_kh012_gt.png}
\\
\bf \begin{turn}{90} 
\bf \ \  Prediction
\end{turn} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/0f1984_kh028_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/1c381f_kh062_pred.png}  &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/2ffa4a_kh062_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/c8b126_kh012_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/d889b1_kh048_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/9aabba_kh012_pred.png}
\\
\\
\end{tabular}
\def\w{0.103\linewidth}
 \centering
\begin{tabular}{c *6c}
\bf \begin{turn}{90} 
\bf \ \ \ \ \ \ \ \   GT
\end{turn} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/8b2ea2_kh056_gt.png}  &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/49e72e_kh005_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/2a8f6b_kh005_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/5db7bc_kh005_gt.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/ab4eb4_kh005_gt.png}  
\\
\bf \begin{turn}{90} 
\bf \ \ Prediction
\end{turn} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/8b2ea2_kh056_pred.png}  &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/49e72e_kh005_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/2a8f6b_kh005_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/5db7bc_kh005_pred.png} &
\includegraphics[height=\w]{source/figures/horizontal_no_trans/ab4eb4_kh005_pred.png}  
\\
\end{tabular}
\caption{
   Results of our population-level scanpath predictions.%, showing that they are aligned well with the ground truth (GT).
}
\label{fig:scanpath_results}
\end{figure*}




% \setlength{\tabcolsep}{1.5pt}
% \def\arraystretch{0.3}% 
% \begin{figure*}[h!]
% \def\w{0.164\linewidth}
%  \centering
% \begin{tabular}{c *9c}
% \bf \begin{turn}{90} 
% \bf \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ GT
% \end{turn} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/0feea2_kh037_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/1a2fc7_kh062_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/6c8b71_kh054_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/46e638_kh028_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/598d81_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/5620ab_kh029_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/ab0c83_kh043_gt.png} &
% \includegraphics[height=\w, trim=10 0 130 10, clip]{source/figures/horizontal_no_trans/5887a5_kh028_gt.png}  &
% \includegraphics[height=\w, trim=55 0 80 0, clip]{source/figures/horizontal_no_trans/a8f275_kh028_gt.png}  
% \\
% \\
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \  Prediction 
% \end{turn} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/0feea2_kh037_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/1a2fc7_kh062_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/6c8b71_kh054_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/46e638_kh028_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/598d81_kh044_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/5620ab_kh029_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/ab0c83_kh043_pred.png} &
% \includegraphics[height=\w, trim=0 0 130 0, clip]{source/figures/horizontal_no_trans/5887a5_kh028_pred.png}  &
% \includegraphics[height=\w, trim=55 0 80 0, clip]{source/figures/horizontal_no_trans/a8f275_kh028_pred.png}
% \\
% \\
% \\
% \\
% \end{tabular}
% \def\w{0.158\linewidth}
%  \centering
% \begin{tabular}{c *9c}
% \bf \begin{turn}{90} 
% \bf \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ GT
% \end{turn} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/ab4d1f_kh037_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/cd9e29_kh005_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/d7cfda_kh012_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/e7a5c0_kh054_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/e18daf_kh012_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/eb06ec_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/f285d7_kh062_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/b4a27a_kh004_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/c6a6d9_kh004_gt.png}
% \\
% \\
% \bf \begin{turn}{90} 
% \bf \ \ \ \ \ \ \ \   Prediction 
% \end{turn} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/ab4d1f_kh037_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/cd9e29_kh005_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/d7cfda_kh012_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/e7a5c0_kh054_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/e18daf_kh012_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/eb06ec_kh044_pred.png} &
% \includegraphics[height=\w]{source/figures/vertical_no_trans/f285d7_kh062_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/b4a27a_kh004_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/c6a6d9_kh004_pred.png}
% \\
% \\
% \\
% \\
% \end{tabular}
% \def\w{0.102\linewidth}
% \begin{tabular}{c *6c}
% \bf \begin{turn}{90} 
% \bf \ \ \ \ \ \ \ \ \  GT
% \end{turn} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/0f1984_kh028_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/1c381f_kh062_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/2ffa4a_kh062_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/c8b126_kh012_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/d889b1_kh048_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/9aabba_kh012_gt.png}
% \\
% \\
% \bf \begin{turn}{90} 
% \bf \ \  Prediction
% \end{turn} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/0f1984_kh028_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/1c381f_kh062_pred.png}  &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/2ffa4a_kh062_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/c8b126_kh012_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/d889b1_kh048_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/9aabba_kh012_pred.png}
% \\
% \\
% \\
% \\
% \end{tabular}
% \def\w{0.103\linewidth}
%  \centering
% \begin{tabular}{c *6c}
% \bf \begin{turn}{90} 
% \bf \ \ \ \ \ \ \ \   GT
% \end{turn} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/8b2ea2_kh056_gt.png}  &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/49e72e_kh005_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/2a8f6b_kh005_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/5db7bc_kh005_gt.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/ab4eb4_kh005_gt.png}  
% \\
% \\
% \bf \begin{turn}{90} 
% \bf \ \ Prediction
% \end{turn} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/8b2ea2_kh056_pred.png}  &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/49e72e_kh005_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/2a8f6b_kh005_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/5db7bc_kh005_pred.png} &
% \includegraphics[height=\w]{source/figures/horizontal_no_trans/ab4eb4_kh005_pred.png}  
% \\
% \end{tabular}
% \caption{
%    Results of our population-level scanpath predictions,
%    showing that they are well aligned with the ground truth (GT).
% }
% \label{fig:scanpath_results}
% \end{figure*}

==> source/07c-FewShots.tex <==

\setlength{\tabcolsep}{0.9pt}
\def\arraystretch{0.2}% 
\begin{figure*}[!]
\def\w{0.12\linewidth}
 \centering
 \begin{tabular}{ccccccccccc}
 & GT & Prediction & GT & Prediction & GT & Prediction & GT & Prediction  & GT & Prediction \\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 1 
\end{turn} & 
\includegraphics[height=\w]{source/figures/supple_results/6c8b71_kh029_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/6c8b71_kh029_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/46e638_kh030_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/46e638_kh030_pred.png}  &
\includegraphics[height=\w]{source/figures/supple_results/449b4f_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/449b4f_kh012_pred.png} & 
\includegraphics[height=\w]{source/figures/supple_results/631068_kh029_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/631068_kh029_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/b44e33_kh035_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/b44e33_kh035_pred.png} 
\\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 2 
\end{turn} & 
\includegraphics[height=\w]{source/figures/supple_results/6c8b71_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/6c8b71_kh037_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/46e638_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/46e638_kh037_pred.png}  &
\includegraphics[height=\w]{source/figures/supple_results/449b4f_kh065_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/449b4f_kh065_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/631068_kh056_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/631068_kh056_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/b44e33_kh058_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/b44e33_kh058_pred.png} 
\\
\end{tabular}






\def\w{0.113\linewidth}
 \begin{tabular}{*7c}
 & GT & Prediction & GT & Prediction & GT & Prediction \\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 1 
\end{turn} & 
\includegraphics[height=\w]{source/figures/supple_results/a09cbe_kh029_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/a09cbe_kh029_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/abe796_kh028_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/abe796_kh028_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/fe14d6_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/fe14d6_kh012_pred.png}
% \includegraphics[height=\w]{source/figures/supple_results/ad1e05_kh012_gt.png} &
% \includegraphics[height=\w]{source/figures/supple_results/ad1e05_kh037_pred.png} 
\\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 2 
\end{turn} & 
\includegraphics[height=\w]{source/figures/supple_results/a09cbe_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/a09cbe_kh065_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/abe796_kh030_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/abe796_kh030_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/fe14d6_kh028_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/fe14d6_kh028_pred.png}
% \includegraphics[height=\w]{source/figures/supple_results/ad1e05_kh048_gt.png} &
% \includegraphics[height=\w]{source/figures/supple_results/ad1e05_kh048_pred.png} 
\\
\end{tabular}






\def\w{0.118\linewidth}
 \begin{tabular}{ccccccccccc}
 & GT & Prediction & GT & Prediction & GT & Prediction & GT & Prediction \\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 1 
\end{turn} & 
% \includegraphics[height=\w]{source/figures/supple_results/b44e33_kh035_gt.png} &
% \includegraphics[height=\w]{source/figures/supple_results/b44e33_kh035_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/c01b8e_kh030_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/c01b8e_kh030_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/c3ac4c_kh028_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/c3ac4c_kh028_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/f9ae9f_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/f9ae9f_kh012_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/27e29a_kh030_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/27e29a_kh030_pred.png}

\\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 2 
\end{turn} & 
% \includegraphics[height=\w]{source/figures/supple_results/b44e33_kh058_gt.png} &
% \includegraphics[height=\w]{source/figures/supple_results/b44e33_kh058_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/c01b8e_kh036_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/c01b8e_kh036_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/c3ac4c_kh058_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/c3ac4c_kh058_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/f9ae9f_kh030_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/f9ae9f_kh030_pred.png} &
\includegraphics[height=\w]{source/figures/supple_results/27e29a_kh036_gt.png} &
\includegraphics[height=\w]{source/figures/supple_results/27e29a_kh035_pred.png}

\\
\end{tabular}






\def\w{0.104\linewidth}
\begin{tabular}{*9c}
 & GT & Prediction & GT & Prediction & GT & Prediction & GT & Prediction  \\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh004_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 1 
\end{turn} & 
\includegraphics[height=\w, trim=10 0 0 0, clip]{source/figures/few-shot/a53761_kh030_gt.png} &
\includegraphics[height=\w, trim=10 0 0 0, clip]{source/figures/few-shot/a53761_kh030_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/b4a27a_kh043_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/b4a27a_kh043_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/bfa4f2_kh004_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/bfa4f2_kh004_pred.png}  &
\includegraphics[height=\w]{source/figures/few-shot/8f9844_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/8f9844_kh012_pred.png} 
\\
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_gt.png} &
% \includegraphics[height=\w]{source/figures/few-shot/168b3b_kh044_pred.png} &
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ \ \ Viewer 2 
\end{turn} & 
\includegraphics[height=\w, trim=10 0 0 0, clip]{source/figures/few-shot/a53761_kh036_gt.png} &
\includegraphics[height=\w, trim=10 0 0 0, clip]{source/figures/few-shot/a53761_kh036_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/b4a27a_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/b4a27a_kh062_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/bfa4f2_kh043_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/bfa4f2_kh043_pred.png}  &
\includegraphics[height=\w]{source/figures/few-shot/8f9844_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/8f9844_kh037_pred.png}  
\\
\end{tabular}
\def\w{0.096 \linewidth}
 \centering
\begin{tabular}{*7c}
 & GT & Prediction & GT & Prediction & GT & Prediction \\
 \bf \begin{turn}{90} 
\bf \ \ \ \  \ \  Viewer 1 
\end{turn} & 
\includegraphics[height=\w]{source/figures/few-shot/5d66d2_kh036_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/5d66d2_kh036_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/5ea384_kh004_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/5ea384_kh004_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/4f4f19_kh004_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/4f4f19_kh004_pred.png} 
\\
\bf \begin{turn}{90} 
\bf \ \ \ \  \ \ Viewer 2 
\end{turn} & 
\includegraphics[height=\w]{source/figures/few-shot/5d66d2_kh037_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/5d66d2_kh037_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/5ea384_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/5ea384_kh062_pred.png} &
\includegraphics[height=\w]{source/figures/few-shot/4f4f19_kh062_gt.png} &
\includegraphics[height=\w]{source/figures/few-shot/4f4f19_kh062_pred.png} 
\end{tabular}
\caption{
%By leveraging a few scanpath samples from each viewer, our model demonstrates the ability to generate personalized scanpaths. Note that we use Viewer 1 and Viewer 2 to show the prediction of two viewers on the same images, but they are not always the same viewers in all the examples.
Scanpaths personalized for two viewers, illustrating our model's ability to generate these by means of only a few scanpath samples from each viewer (note that ``Viewer 1'' and ``Viewer 2'' are generic terms; the viewers are not the same across all examples).
}
\label{fig:fewshot_results}
\end{figure*}



==> source/07d-Algorithm.tex <==

\begin{algorithm}[t]
 % \caption{RL for Scanpath Prediction}
  
  \begin{algorithmic}[1]
    \State Initialize policy model $\pi_{\theta}$ parameterized by $\theta$
    \State Initialize reward function $R_{DTW}$, $R_{sal}$

    \State{\textbf{For \textit{each training step}, do}}
    \State \qquad Initialize empty list of sampled points $\hat{p}$, predicted points $p^{pred}$, salient-value rewards list $\hat{r}_{sal}$, $r^{pred}_{sal}$
    
    \State \qquad{\textbf{For \textit{each step}~$i$, do}}
    % \FOR{\textit{each step}~$i$}
      \State \qquad\qquad  Sample  images $\image$, ground-truth $p$,  saliency maps $M_{sal}$
      \State \qquad\qquad  Generate mean, variance of points' Gaussian distribution: 
      $$\mu_i, \sigma_i \gets \text{forward}(\image, \hat{p}_{:i-1}, \theta)$$
      \State \qquad\qquad  Sample predicted points from the Gaussian distribution:
      $$\hat{p}_i \gets \text{sample}(\mu_i, \sigma_i)$$
      \State \qquad\qquad  Generate mean of the Gaussian distribution for points:
      $$\mu^{pred}_i \gets \text{StopGradient}(\text{forward}(\image, p^{pred}_{:i-1}, \theta))$$
      \State \qquad\qquad  Compute salient-value rewards for each sampled point: 
      $$\hat{r}_{sal,i} \gets R_{sal}(\hat{p}_i, M_{sal})$$
      \State \qquad\qquad  Compute salient-value rewards for each predicted point: 
      $$r^{pred}_{sal,i} \gets R_{sal}(p^{pred}_i, M_{sal})$$
        
      \State \qquad\qquad  Add $\hat{p}_i$ to set $\hat{p}$; and add $\hat{r}_{sal,i}$ to set $\hat{r}_{sal}$ 
      \State \qquad\qquad  Add $\mu^{pred}_i$ to set $p^{pred}$; and add $r^{pred}_{sal,i}$ to set $r^{pred}_{sal}$

    \State \qquad\textbf{end for}
    
    \State \qquad Compute DTW rewards for all sampled and predicted points: 
      $$\hat{r}_{DTW} \gets -R_{DTW}(\hat{p}, p); \;
      r^{pred}_{DTW} \gets -R_{DTW}(p^{pred}, p)$$
      \State \qquad Compute total rewards of sampled and predicted points:
     $$\hat{r} \gets \hat{r}_{DTW} + \text{discount}(\hat{r}_{sal}); \;
     r^{pred} \gets r^{pred}_{DTW} + \text{discount}(r^{pred}_{sal})$$
    
    \State \qquad Compute advantages: $A \gets \hat{r} - r^{pred}$
      \State \qquad Compute loss gradient with respect to model parameters: $$\nabla_\theta \gets \text{{compute\_gradient}}(\pi_{\theta}(\hat{p}), A)$$
      \State \qquad Update model parameters using gradient ascent: $\theta \gets \theta + \alpha \nabla_\theta$

      \State \textbf{end for}
  \end{algorithmic}
  \caption{A comprehensive description of the RL approach proposed for scanpath prediction -- an algorithm to optimize the scanpath-prediction process iteratively, with feedback from salient-value and DTW rewards employed to enhance performance}
  \label{algo:rl}
\end{algorithm}



==> source/07e-saccade_figure.tex <==

\begin{figure}[t]
    \centering
    \def\w{0.18\linewidth}
    \captionsetup[subfloat]{labelformat=empty}
    \subfloat[\textbf{Ground Truth}]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_overall_ground_truth.png}
    }
    \hfill
    \subfloat[Itti-Koch]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_Itti-Koch-based_overall.png}
    }
    \hfill
    \subfloat[DeepGaze III]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_DeepGazeIII_overall.png}
    }
    \hfill
    \subfloat[DeepGaze++]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_DeepGaze++_overall.png}
    }
    \hfill
    \subfloat[PathGAN Pretrained]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_PathGAN_Pretrained_overall.png}
    }
    \hfill  \\
    \subfloat[]{\phantom{\includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_PathGAN_UEyes_overall.png}}}
      \hfill
    \subfloat[PathGAN (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_PathGAN_UEyes_overall.png}
    }
    \hfill 
    \subfloat[PathGAN++ (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_PathGAN++_overall.png}
    }
    \hfill
    \subfloat[SaltiNet (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_SaltiNet_overall.png}
    }
    \hfill
    \subfloat[UMSS (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_UMSS_overall.png}
    }
    \hfill \\
    \subfloat[]{\phantom{\includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_PathGAN_UEyes_overall.png}}}
      \hfill
    \subfloat[ScanGAN (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_ScanGAN_overall.png}
    }
    \hfill
    \subfloat[ScanDMM (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_ScanDMM_overall.png}
    }
    \hfill
    \subfloat[Chen et al. Method (UEyes)]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_ScanVQA_overall.png}
    }
    \hfill
    \subfloat[\textbf{Our Method}]{
        \includegraphics[width=\w]{source/figures/scanpath_direction_plots/direction_RL_overall.png}
    }
    \hfill
    
     \caption{Plots of ground-truth and predicted gaze directions. Analyzing saccade bias yields insight related to directions and distances between consecutive fixation points. For instance, real-world gaze directions' convergence predominantly near the right and bottom of the images, with greater distances observed particularly toward the right, suggests a preference for directing the gaze from left to right (with fairly large motions) and from top to bottom. Our model captures this property better than others do.}
    \label{fig:predict_saccade_direction}
\end{figure}


==> source/07f-visited_revisited_figure.tex <==
\begin{figure}[t]
    \centering
    \def\w{0.18\linewidth}
    \captionsetup[subfloat]{labelformat=empty}
    \subfloat[\textbf{Ground Truth}]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/Ground_Truth_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[Itti-Koch]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/Itti-Koch_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[DeepGaze III]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/DeepGazeIII_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[DeepGaze++]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/DeepGaze++_visit_resvisit_overall.png}
    } \hfill
    \subfloat[PathGAN Pretrained]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/PathGAN_Pretrained_visit_resvisit_overall.png}
    }
    \hfill    \\
    \subfloat[]{\phantom{\includegraphics[width=\w]{source/figures/visited_revisited_plots/PathGAN_UEyes_visit_resvisit_overall.png}}}
      \hfill
    \subfloat[PathGAN (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/PathGAN_UEyes_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[PathGAN++ (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/PathGAN++_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[SaltiNet (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/SaltiNet_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[UMSS (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/UMSS_visit_resvisit_overall.png}
    }
    \hfill  \\
    \subfloat[]{\phantom{\includegraphics[width=\w]{source/figures/visited_revisited_plots/PathGAN_UEyes_visit_resvisit_overall.png}}}
      \hfill
    \subfloat[ScanGAN (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/ScanGAN_visit_resvisit_overall.png}
        }
    \hfill
    \subfloat[ScanDMM (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/ScanDMM_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[Chen et al. Method (UEyes)]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/ScanVQA_visit_resvisit_overall.png}
    }
    \hfill
    \subfloat[\textbf{Our Method}]{
        \includegraphics[width=\w]{source/figures/visited_revisited_plots/ours_visit_resvisit_overall.png}
    }
    \hfill
     \caption{For each scanpath-prediction model, the percentage of the elements of each type visited and revisited. Of the models evaluated, ours produces the estimation closest to the ground truth. 
      {The ``Visited'' figure is calculated from % FYI: Since this must be multiplied by 100, `from' rather than `by'. als
dividing the count of visited elements by the number of elements belonging to the element-type class in question, across all GUI images. 
     An element is considered revisited when receiving at least two non-consecutive fixations in the sequence.}
     }
    \label{fig:visit-results}
\end{figure}



==> source/07g-IndividualResults.tex <==
\setlength{\tabcolsep}{0.9pt}
\def\arraystretch{0.2}% 
\begin{figure*}[!]
\def\w{0.138\linewidth}
 \centering
 \begin{tabular}{cccccc}
  &  User 1 & User 2  & User 3 &  User 4    \\
   \begin{turn}{90} 
\ \ \ \  Ground Truth
\end{turn} & 
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh012_gt.png} &
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_gt.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh030_gt.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_gt.png}
\\
 \begin{turn}{90} 
 \ \ \ \  \ \ \ Prediction
\end{turn} & 
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh012_pred.png} &
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_pred.png}
&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh030_pred.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_pred.png}
\\
\\
  & User 5 & User 6 & User 7 & User 8    \\
 \begin{turn}{90} 
 \ \ \ \   Ground Truth
\end{turn} & 
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh028_gt.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh036_gt.png}
&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh037_gt.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_gt.png}
\\
\begin{turn}{90} 
 \ \ \ \  \ \ \ Prediction
\end{turn} & 
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh028_pred.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh036_pred.png}
&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh037_pred.png}&
\includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_pred.png}&
\includegraphics[height=\w]{source/figures/colormap.png}
\end{tabular}
\caption{
Example scanpath predictions for several distinct viewers.
}
\label{fig:individual}
\end{figure*}




% \setlength{\tabcolsep}{0.9pt}
% \def\arraystretch{0.2}% 
% \begin{figure*}[!]
% \def\w{0.145\linewidth}
%  \centering
%  \begin{tabular}{cccccc}
%   & GT & Prediction & & GT & Prediction   \\
%   \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 1 
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh012_gt.png} &
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh012_pred.png} &
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 2 
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_pred.png}
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh012_gt.png} &
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh012_pred.png}
% \\
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 3 
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh030_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh030_pred.png}&
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 4 
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_pred.png}
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh030_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh030_pred.png}
% \\
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 5
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh028_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh028_pred.png}&
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 6
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh036_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh036_pred.png}
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh029_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh029_pred.png}
% \\
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 7 
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh037_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh037_pred.png}&
% \bf \begin{turn}{90} 
% \bf \ \ \ \  \ \ \ \ User 8
% \end{turn} & 
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_gt.png}&
% \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_pred.png}
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh037_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh037_pred.png}
% \\
% % \bf \begin{turn}{90} 
% % \bf \ \ \ \  \ \ \ \ User 5
% % \end{turn} & 
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh035_pred.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh054_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh054_pred.png}
% % \\
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh056_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh056_pred.png}
% % \\
% % \bf \begin{turn}{90} 
% % \bf \ \ \ \  \ \ \ \ User 7 
% % \end{turn} & 
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh048_pred.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh005_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh005_pred.png}
% % \\
% % \bf \begin{turn}{90} 
% % \bf \ \ \ \  \ \ \ \ User 8 
% % \end{turn} & 
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/0f1984_kh058_pred.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh065_gt.png}&
% % \includegraphics[height=\w]{source/figures/individual_results/5db7bc_kh065_pred.png}
% \\
% \end{tabular}

% \caption{
% Example scanpath predictions for several distinct viewers.
% }
% \label{fig:individual}
% \end{figure*}


==> source/1104-Results-old.tex <==
\section{Experiments}
%\input{source/07d-Algorithm}

In this section, we conduct experiments for both population-level and individual-level prediction.


% \begin{figure}[h]
%   \def\w{\linewidth}
%   \centering

%  \includegraphics[width=\w]{source/figures/scanpath_length_distribution.png}

% \caption{\ADD {The distribution of scanpath lengths for the eye-tracking-based dataset UEyes. With an average scanpath length of 15.3 points, the visualization highlights that most scanpaths are clustered around length 15.}}
%   \label{fig:scanpath_length_distribution}
% \end{figure}


\subsection{Dataset}

We utilized the \textit{UEyes} dataset~\cite{jiang2023ueyes}, which comprises 1,980 images, from four common types of GUI (posters, desktop user interfaces, mobile ones, and webpages), with eye-tracking data collected from 62 participants. 
This dataset was meticulously compiled by means of a high-fidelity eye tracker in a laboratory setting, so as to guarantee precise coordinates in the \emph{XY} plane, and the coordinate values were subjected to participant-specific calibration accounting for factors such as eye--display distance.
%Throughout the data-collection process, the screen angle for each participant was checked and adjusted, for emulation of the individual-specific typical viewing scenario. Each participant, seated between roughly 50 and 65 centimeters from the screen, experienced the same visual angle for all four types of user interface. Uniformity of visual angle was enforced for ease of comparison across interface types: all data collection and subsequent analysis adhered to this method consistently. 
%By guaranteeing that the limits to the tracking technology's accuracy cannot unduly influence assessment of the mobile-device user interfaces, the uniform presentation strategy maintains fairness in the evaluation process. 
%Fixation duration was ascertained directly from the timings recorded by the eye tracker.
%The participant free-viewed each GUI for seven seconds.
We have used the same training/test GUI image split that~\citet{jiang2023ueyes} did, dividing the set such that 1,872 images were placed in the training set and 108 in the test set while making sure that the four GUI types were distributed evenly in each set.
In addition, to establish a training/test split for individual-level prediction, we employed a further procedure: randomly assigning 53 users to the training set (85\%) and the remaining 9 to the test set (15\%). 
Our model was trained on the gaze data collected from when the training users looked at the GUIs in the set of training images. We present more details of the dataset and implementation in the Supplementary Materials.
%~\autoref{fig:scanpath_length_distribution} presents the distribution of scanpath lengths from the UEyes dataset.}



%\input{source/07a-ComparisonFigures}


% \subsection{Implementation Details}

% \begin{add}
% \subsubsection{{Algorithm}}

% Algorithm \ref{algo:rl}'s pseudocode comprehensively describes our suggested RL-based approach to training the scanpath-prediction model. This algorithm is designed to optimize the prediction process iteratively by taking advantage of feedback from salient-value and DTW rewards to enhance performance. The algorithm progresses through the following six stages:

% \begin{enumerate}
% \setlength{\itemsep}{0pt}
% \item \textbf{Generating the Policy Model's Output}: In each iteration, % FYI: This is a bit safer since there are six `steps'. -als
% the algorithm generates the model output, comprising the mean and variance of a Gaussian distribution. This distribution informs the sampling of points, and its mean values function as the predicted points.
    
%     \item \textbf{Computing the Salient-Value Reward}: The algorithm computes a salience reward for each iteration's sampled and predicted points. This reward reflects the importance of the points with reference to the overall saliency map.

%     \item \textbf{Constructing Scanpaths}: The sampled and predicted points from each iteration are added to two empty sets, forming the sampled and predicted scanpath as the algorithm progresses.

%     \item \textbf{Calculating the DTW Reward}: The algorithm calculates the dynamic time warping reward for the sampled and predicted scanpath, comparing it with the ground-truth scanpath. As a metric for similarity between two sequences, DTW aids in assessing how well the predicted and real-world scanpath match.

%     \item \textbf{Computing the Total Reward}: Total reward values are computed by combining the salient-value rewards and DTW rewards. These rewards are usually discounted, to give greater weight to recent predictions.

%     \item \textbf{Updating the Policy}: Finally, the algorithm updates the policy derived from the reward. This step involves adjusting the model's parameters or the strategy behind sampling and predicting of points. The goal is to optimize the algorithm's performance for accurate scanpath predictions.
% \end{enumerate}
% \end{add}

% \subsubsection{{Training Process}}



% \ADD{Our decision to implement the vision encoder by means of the ViT-Base~\cite{Dosovitskiy2020ViT} architecture, with the aforementioned 12-layer version of the model, was driven by its demonstrated ability to handle diverse visual patterns and its potential to outperform traditional convolutional neural networks in various task conditions. By means of self-attention and Transformer-based mechanisms, the ViT-Base model can learn intricate relationships among image elements without requiring handcrafted architecture-level modifications for specific problem domains.}
% Before feeding an image to the vision encoder, we resized it to a square with dimensions of $w_\textrm{inp}=h_\textrm{inp}=256$, divided that square into $256$ patches each of size $16\times 16$, and embedded these with a dimensionality of $d_{\image}=768$. 
% For the fixation decoder, we employed a three-layer Transformer, utilizing the first three BERT-Base~\cite{devlin2019bert} layers. % I can't readily verify this usage vs. `BERT base', `BERT Base', `BERT[Base]', ...  -als

% To mitigate the policy-gradient-associated training variance, we took a two-part approach to the training.
% The process initializes the mean $\mu_i$ and variance $\sigma_i$ of the Gaussian distribution $\pi_{\theta}(\hat{p}i)$ for fixation points by minimizing the 
% result for the following objective function: % NB: Or this might mean `objective function's value thus:'? -als
% \begin{flalign}
% \loss(\theta) = \sum_{i=1}^T [(\sigma_i - \sigma_{p_i})^2 + (\mu_i-p_i)^2 ],
% \end{flalign}
% where $p_i=(x_i,y_i,t_i)$ represents the ground-truth fixations and the hyper-parameters $\sigma_{p_i}=(\sigma_{x_i}, \sigma_{y_i},\sigma_{t_i})$ are predefined and adjusted on the basis of the image dimensions, while $\sigma_{t_i}$ is fixed at 0.1,
% in keeping with a normalized viewing angle of five degrees. 
% This initialization process entails 30 training epochs with a batch size of 64 and a learning rate of $10^{-4}$.
% The second step employs policy-gradient techniques to train the policy further within an RL framework, utilizing DTW and salient-value rewards. This step applies 20 training epochs with a batch size of 64 and a learning rate of $10^{-5}$. The policy model is optimized via policy gradients to generate a sequence of $T=15$ points as the final output. \ADD{This setting for $T$ accounts for the fact that many methods~\cite{itti1998model, kummerer2022deepgaze, jiang2023ueyes, wang2023scanpath, Assens2018pathgan} rely on a fixed number of generated points, with metrics' results depending considerably on the lengths.
% A value of 15 is consistent with the concentration of scanpath lengths around this value, captured in ~\autoref{fig:scanpath_length_distribution}.
% }






\input{source/06a-quantitative_table}




\subsection{Population-Level Scanpath Prediction}





To assess how well our model, when given an input GUI image, predicts the spatiotemporal information of scanpaths, we compared its performance with that of several scanpath models: the Itti--Koch model with IOR~\cite{itti1998model}, DeepGaze~III~\cite{kummerer2022deepgaze}, DeepGaze++~\cite{jiang2023ueyes},
SaltiNet~\cite{assens2017saltinet}, the UMSS system~\cite{wang2023scanpath}, PathGAN~\cite{Assens2018pathgan},  PathGAN++~\cite{jiang2023ueyes},
ScanGAN~\cite{martin2022scangan360}, 
ScanDMM~\cite{Sui_2023_CVPR},
and ~\citet{chen2021predicting}. For a fair comparison, we trained all the learning-based models on the UEyes dataset with the same training/test split. 



\subsubsection{{Qualitative Evaluation}}

\begin{add}
Qualitative comparison revealed that the predictions made by our model lie closer to the ground-truth values than the other models. \autoref{fig:scanpath_qualitative} summarizes this comparison of all the models.  
We found that, while PathGAN++ and ScanGAN trained on UEyes, thanks to their discriminative component, excel at generating realistic trajectories, the points they predict often fall outside the salient areas. In addition, PathGAN++ tends to produce clusters in local areas and exhibits a bias toward the center of the GUI images. 
In contrast, DeepGaze++ performs well in locating fixation points by applying post-processing techniques to their density maps. Nevertheless, it generates fixations in incorrect order; on account of the non-differentiable nature of the post-processing, the order is not optimized in line with the ground-truth data.
The Itti--Koch-based, SaltiNet, and UMSS generate scanpaths from saliency maps, encouraging fixations that lie in salient areas. Still, these models often produce an incorrect sequence for the fixation points since they do not optimize for correct fixation order. 
Chen et al., in turn, tends to generate several clusters of closely grouped points.
This tendency arises from the fact that their approach to the integration of RL places considerable emphasis on precision in the prediction of fixations while overlooking the need to spread consecutive points out more.
Finally, ScanDMM appears to focus relatively strongly on text elements. %This characteristic is analyzed further in ~\autoref{sec:visit}.
Our model assigns fixation points to salient areas and attends to the points' order with greater precision.
It accomplishes this by utilizing the salient-value reward ($r_\mathrm{sal}$) to emphasize points that lie within areas of interest and by employing the DTW reward ($r_\mathrm{dtw}$) to encourage more accurate trajectories.
More results are shown in the Supplementary Materials.
%\autoref{fig:scanpath_results} presents further population-level prediction results showcasing the performance of our model. 
\end{add}


\input{source/06b-ablation-table}


\def\arraystretch{1}% 
\begin{table*}[t]
\scalebox{0.9}{\setlength\tabcolsep{5pt}
\begin{tabular}{lcccccccccc}
\hline
\multirow{ 2}{*}{\textbf{Model}}  & \multirow{ 2}{*}{\textbf{DTW} $\downarrow$}  & \multirow{ 2}{*}{\textbf{TDE} $\downarrow$} & \multirow{ 2}{*}{\textbf{Eyenalysis} $\downarrow$} & \multirow{ 2}{*}{\textbf{DTWD} $\downarrow$} & \multicolumn{6}{|c}{\textbf{MultiMatch} $\uparrow$}  \\
 &  &  &   & &  \multicolumn{1}{|c}{\textbf{Shape}}   & \textbf{Direction}  &  \textbf{Length}   & \textbf{Position}   & \textbf{Duration}  & \textbf{Mean}  \\
\hline
\bf Population-Level &   4.082 $\pm$  1.124    &  \bf 0.121  $\pm$  0.028   &   \bf 0.035  $\pm$  0.017   &    5.054  $\pm$  1.088 &   0.942    &  \bf 0.748    &  \bf  0.940   &   0.825   &    0.750   &  0.841    \\
\hline
\bf Individual-Level &   \bf  4.058 $\pm$  1.135   &   \bf 0.121  $\pm$  0.029   &   0.036  $\pm$  0.017   & \bf   4.996  $\pm$  1.078 &  \bf  0.944    &  0.747   &   \bf  0.940   &    \bf  0.826   &   \bf  0.754   & \bf   0.842    \\
\bottomrule
\end{tabular}
}
\caption{
    We compare the personalized scanpaths against the general ones to quantify the effectiveness in capturing the characteristics of individual users.
}
\label{tbl:individual_table}
\end{table*}


\subsubsection{{Quantitative Evaluation}}

We assessed the models' performance via commonly employed metrics for scanpath evaluation~\cite{anderson2015comparison, fahimi2021metrics}. 
To account for variations in image sizes and minimize discrepancy-related errors, 
we normalized the fixation points' coordinates to the $[0,1]$ range.
For metrics to address fixations' position and temporal order, we examined DTW,
% \cite{berndt1994using, salvador2007toward} % FYI: I've removed redundancy. -als
time delay embedding (TDE)~\cite{tim1991embedology, wang2011simulating}, and Eyenalysis~\cite{mathot2012eyenalysis}.
In addition, we extended DTW to encompass duration; DTWD enables considering the points' positions and duration. The optimal alignment for DTWD is computed based on position, and then the error is computed based on duration as well
Finally, MultiMatch~\cite{dewhurst2012depends} permitted us to assess numerous aspects of 
scanpaths, including shape, direction, length, position, and duration.
%
\autoref{tbl:scanpaths_quantitative} presents a comprehensive comparison encompassing all of these metrics. 
To guarantee a fair assessment in light of the path-length issue noted earlier in the paper, we standardized the predicted scanpaths from all the models to contain no more than 15 fixation points.
Our model outperforms the baseline models by every metric, with the exception of TDE and MultiMatch for \texttt{Shape}. 
Its superiority to the other models when evaluated via the DTW and Eyenalysis metrics 
indicates that our model simulates scanpath trajectories more realistically. 
Among the preexisting models considered, only PathGAN, PathGAN++, SaltiNet, UMSS, and the Chen team's model are able to predict temporal information. 
While the first two of these are available in two versions, one with gaze-duration prediction and one without, it is evident from our results that additionally predicting temporal information actually leads to reduced scanpath-prediction accuracy on both models' part. 
Our model excels by the DTWD and MultiMatch \texttt{Duration} metrics, 
further attesting to its capacity to yield more accurate results. 
It outperforms even versions that include prediction of temporal information.



\subsubsection{Ablation Study}


\autoref{tbl:scanpaths_ablation} presents the results from an ablation study for utilizing RL to produce both population- and individual-level scanpaths. 
The results reveal that Transformer-only (`w/o RLs') does not produce satisfactory results: incorporating RL greatly enhances the prediction of fixations and their duration.
With its population-level prediction, our RL model brings an improvement of 14.7\% and 26.5\% by the TDE and Eyenalysis metrics, respectively. 
This is evidence that using RL increases the model's capacity to generate realistic fixations for scanpaths.
As for duration, applying RL has a positive influence on prediction accuracy, demonstrated by the 4.8\% improvement shown by the DTWD.
Similar effects are visible with the individual-specific predictions connected with training users (i.e., the trained model's prediction of scanpaths for GUI images when given the IDs of particular training users). 
Additionally, the results highlight that the absence of either each type of reward or of inhibition of return leads to a decline in overall accuracy.












% \begin{add}


% \subsubsection{Scanpath Properties}
% \input{source/07e-saccade_figure}
% \input{source/07f-visited_revisited_figure}




% Analyzing scanpath properties facilitates comparing scanpath-prediction models at another level. Accordingly, we address two key facets of scanpaths below: 1) saccade angle and amplitude distribution and 2) visited- and revisited-element ratios. All results shown here were evaluated by means of the test data. 






% \paragraph{\textbf{Saccade Angle and Amplitude Distribution}}


% \autoref{fig:predict_saccade_direction} characterizes the saccade-angle and amplitude-distribution aspect of our comparison.   
% Visualizations of saccade bias assist in examining the direction and distance traveled between successive fixation points. Researchers have observed that the ground-truth gaze directions predominantly lie toward the right and % `and/or'? -als
% the bottom portion(s) % Or just `portion' if this doesn't refer to discrete elements. -als
% of the GUIs, with the distances being greater toward the right-hand side. This is evidence that users tend to move their gaze left--right (rather than the opposite) across large distances and from top to bottom. Our model excels at capturing and replicating said characteristic, and it outperforms preexisting models in this regard. 
% The pretrained PathGAN model and DeepGaze III's distributions manifest clustering, caused primarily by the presence of point clusters in the predicted scanpaths.
% Both PathGAN models trained on UEyes and PathGAN++ suffer from an incorrect center bias in their distributions.
% This limitation is evident also in the ScanGAN and ScanDMM models, as their distributions' middle-centricity attest.
% Furthermore, the Chen et al. model exhibits a tendency to place consecutive fixations in close mutual proximity.
% The Itti--Koch-based one and DeepGaze++, by incorporating IOR, prevent short distances between successive fixation points.
% Consequently, both output larger saccade amplitudes than those visible in the ground-truth data, thereby showing a weakness of their approach to capturing natural gaze behavior. 
% SaltiNet and UMSS are similar in this respect, with the shortcoming being evident from the extent of the movement distance.
% Though employing inhibition of return, our model still generates some short vertical-movement distances.



% \paragraph{\textbf{Visited- and Revisited-Element Ratios}}
% \label{sec:visit}
% To enable comparing the visited- and revisited-element ratios in the various models' scanpaths for people looking at GUIs, 
% we performed segmentation and classified the interface elements into three distinct categories: images, text, and faces. 
% Then, we calculated the number of elements in each category that were visited (fixated on) and revisited (fixated upon at least once more), where an element already visited is considered revisited if encompassing at least three fixation points after a fixation on a different element.
% The results of our comparison are presented in~\autoref{fig:visit-results}. 
% %
% Among the models evaluated, ours produces the estimation nearest the ground truth for both visited- and revisited-element ratios. 
% The other models' performance varies greatly, with some scanpaths representing underestimation of these ratios and others leading to overestimation.
% For instance, both the visiting and the revisiting ratios from the pretrained PathGAN and DeepGaze III models' output are unrealistically low. 
% While SaltiNet and UMSS perform well at accurately representing visiting and revisiting ratios for images, these ratios are still too low for text and faces. 
% The Itti--Koch-based model captures both ratios well for text in addition to images, but its performance is less good for faces, with excessively low revisit ratios. 
% Conversely, DeepGaze++'s predictions match the ground-truth visit ratios excellently while the revisit ratios are too high.
% Both ScanGAN and ScanDMM yield excessively high revisit ratios for text, with ScanDMM's predictions simultaneously representing an underestimation for revisiting faces.
% Also, this analysis supports our observation in the qualitative comparison that ScanDMM is more text-focused. 
% Finally, the model by Chen and colleagues generates predictions that can be characterized as underestimating the revisited-element ratio for both text and faces while overestimating the visited-element ratio for faces.
% %Overall, our model provides for the most accurate estimation of visited- and revisited-


% \end{add}


\subsection{Individual-Level Scanpath Prediction}


% \begin{figure*}[t]
% \def\w{0.26\linewidth}
%  \centering
% \begin{tabular}{*3c}
% \includegraphics[height=\w]{source/figures/sample_dtw.png} &
% \includegraphics[height=\w]{source/figures/sample_tde.png} &
% \includegraphics[height=\w]{source/figures/sample_eyenalysis.png}
% \end{tabular}
% \caption{\ADD{
% Performance for individual-level scanpath prediction plotted against sample quantity. 
% As the sample count rises, the quantitative outcome (as measured by DTW, TDE, and Eyenalysis) improves. A noteworthy pattern is detectable for the span between as few as 10 samples and about 50, with all three panes likewise showing a clear deceleration in advancement as the sample count climbs to 70 or more (this is particularly evident with the DTW and TDE metrics). 
% }
% }
% \label{fig:sample}
% \end{figure*}



% \input{source/07g-IndividualResults}

The challenge of predicting personalized individual-level scanpaths for unknown users has not been addressed in prior research. While training directly with a large quantity of data for the relevant user would yield greater similarity with the ground truth, full retraining for each new user, with more data, is impractical. Our model achieves a workable balance by generating scanpaths tailored to each user's viewing behaviors and idiosyncrasies while still permitting a single model's application for all users, without the burden of retraining.
We verified our model's ability to generate personalized scanpaths by proceeding from a few scanpath samples from the individual, thus confirming that 
the model can effectively capture each user's viewing preferences/behaviors and reflect them in its output.

When encountering a test user with a few samples available, the model updates the user embedding by utilizing a set of $n_\mathrm{path}$ scanpaths obtained from that user (in our experiments, $n_\mathrm{path}=50$). 
The process involves updating the learnable vector (i.e., the user embedding) by freezing other parts of the network and backpropagating from the scanpath samples, thereby allowing each user's distinct viewing behaviors to be encoded in a separate embedding space.
Once the model has updated user embedding, it can predict scanpaths specific to this unique user, thereby customizing its predictions for this individual's viewing behaviors.

\autoref{fig:fewshot_results} presents individual-level scanpath prediction in qualitative terms by way of a few examples. Since there is currently no established baseline method that can serve as a comparison point for our proposed approach, we compare the personalized scanpaths against the general scanpaths to quantify the effectiveness in capturing the characteristics of individual users (\autoref{tbl:individual_table}). We provide more results and explain the relationship between sample quantity and the performance in the Supplementary Materials.








==> source/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip

